Allocation of Heterogeneous Resources in General Lotto Games

The allocation of resources plays an important role in the completion of system objectives and tasks, especially in the presence of strategic adversaries. Optimal allocation strategies are becoming increasingly more complex, given that multiple heterogeneous types of resources are at a system planner's disposal. In this paper, we focus on deriving optimal strategies for the allocation of heterogeneous resources in a well-known competitive resource allocation model known as the General Lotto game. In standard formulations, outcomes are determined solely by the players' allocation strategies of a common, single type of resource across multiple contests. In particular, a player wins a contest if it sends more resources than the opponent. Here, we propose a multi-resource extension where the winner of a contest is now determined not only by the amount of resources allocated, but also by the composition of resource types that are allocated. We completely characterize the equilibrium payoffs and strategies for two distinct formulations. The first consists of a weakest-link/best-shot winning rule, and the second considers a winning rule based on a weighted linear combination of the allocated resources. We then consider a scenario where the resource types are costly to purchase, and derive the players' equilibrium investments in each of the resource types.

==> WC_proof.tex <==
\subsection{Proof of Proposition \ref{thm:WC}}

We establish a series of Lemmas to establish Theorem \ref{thm:WC} in a similar manner to Theorem \ref{thm:WL}. For the weighted contribution winning rule, we consider the multi-resource game $\ML(\bX,\bY; W_\WC,\bv)$, where $W_\WC$ is defined in \eqref{eq:WC} with effectiveness parameters $\bs{a}$ and $\bs{b}$. Similar to the approach for the proof of Theorem \ref{thm:WL}, we study the class of weakest-link strategies $\F_\WL(\bX)$ for player $\mcx$ (Definition \ref{def:CAS_X}). However, here we also consider weakest-link strategies $\F_\WL(\bY)$ for player $\mcy$ as well.

The following Lemma establishes an upper bound on player $\mcx$ for any $\hat{F}_\mcy \in \F_\WL(\bY)$.
\begin{lemma}\label{lem:UB_WC}
    Consider $\ML(\bX,\bY;W_\WC,\bv)$. Suppose $\hat{F}_\mcy \in \F_\WL(\bY)$ is a strategy of the form \eqref{eq:CAS_X}. Then it holds that for any $F_\mcx \in \F(\bX)$,
    \be
        \pi_\mcx(F_\mcx,\hat{F}_\mcy) \leq \UB_\WC(\dy)
    \ee
    where $\dy \in [0,1]$ is the parameter of $\hat{F}_\mcy$, and
    \be
    	\UB_\WC \triangleq 1 - \dy + \frac{\dy^2}{2 \beta(\bX,\bY)}
    \ee
    where $\beta$ is defined in Theorem \ref{thm:WC}.
\end{lemma}

\begin{proof}
	For any $F_\mcx \in \F(X)$, we have that the payoff in contest $c$ is
	\be
		\ba
			&\pi_{\mcx,c}(F_{\mcx,c},\hat{F}_{\mcy,c}) =\E_{F_{\mcx,c}, \hat{F}_{\mcy,c}}\left[\ones\left\{ \sum_{t\in\mct} a_t x_{c,t} \geq  \sum_{t\in\mct} b_t y_{c,t} \right\} \right] \\
			&= \E_{F_{\mcx,c}}\left[ \P\left( \bar{y}_c \leq \sum_{t\in\mct} a_t x_{c,t} \right) \right] \\
		\ea
	\ee
	where $\bar{y}_c := \sum_{t\in\mct} b_t y_{c,t}$ is the random variable defined as the weighted sum of allocations to contest $c$. The cumulative distribution of $\bar{y}_c$ is given by
	\be
		\bar{F}_{\mcy,c}(u) := 1 - \dy + \dy\min\left\{ \frac{\dy}{2v_c \sum_{t\in\mct} b_t Y_t}\cdot u , 1 \right\}
	\ee
	for any $u\geq 0$. We then get
	\be
		\ba
			&\pi_{\mcx,c}(F_{\mcx,c},\hat{F}_{\mcy,c}) =\E_{F_{\mcx,c}}\left[\bar{F}_{\mcy,c}\left(\sum_{t\in\mct} a_t x_{c,t} \right) \right] \\
			&= 1 - \dy + \dy\cdot \E_{F_{\mcx,c}}\left[\min\left\{ \frac{\dy \sum_{t\in\mct} a_t x_{c,t} }{2v_c \sum_{t\in\mct} b_t Y_t}, 1 \right\} \right] \\
			&\leq 1 - \dy + \dy\cdot \E_{F_{\mcx,c}}\left[ \frac{\dy \sum_{t\in\mct} a_t x_{c,t} }{2v_c \sum_{t\in\mct} b_t Y_t} \right] \\
			&= 1 - \dy + \dy\cdot \frac{\dy \sum_{t\in\mct} a_t \cdot \E_{F_{\mcx,c}}[x_{c,t} ] }{2v_c \sum_{t\in\mct} b_t Y_t}  \\
		\ea
	\ee
	Now, observe that the total payoff can be written
	\be
		\ba
			&\pi_\mcx(F_\mcx,\hat{F}_\mcy) = \sum_{c\in\mcc} v_c \cdot \pi_{\mcx,c}(F_{\mcx,c},\hat{F}_{\mcy,c}) \\
			&\leq 1 - \dy + \frac{\dy^2}{2 \sum_{t\in\mct} b_t Y_t}\cdot \sum_{c\in\mcc} \sum_{t\in\mct}  a_t \cdot \E_{F_{\mcx,c}}[x_{c,t} ]  \\
			&\leq 1 - \dy + \frac{\dy^2}{2}\cdot \frac{\sum_{t\in\mct}  a_t X_t}{ \sum_{t\in\mct} b_t Y_t}  \\
%			&=  1 - \dy + \frac{\dy^2}{2}\cdot \beta(\bX,\bY)
		\ea
	\ee
	where the last inequality follows from $F_\mcx \in \F(\bX)$ \eqref{eq:ML_admissible}.
\end{proof}

The next Lemma provides the smallest upper bound that player $\mcy$ can impose by using strategies $\hat{F}_\mcy$ of the form \eqref{eq:CAS_Y}.
\begin{lemma}\label{lem:min_UB_WC}
	Consider $\ML(\bX,\bY;W_\WC,\bv)$. Then,
	\be\label{eq:UB_OPT_WC}
		\min_{\dy \in [0,1]  } \UB_\WC(\dy) = L(\beta(\bX,\bY)).
	\ee
	The strategy $F_\mcy^* \in \F_\WL(\bY)$ that imposes the bound upper bound  $L(\beta(\bX,\bY))$ is given as follows. 
	If $\beta(\bX,\bY) \leq 1$, then
    	\be
       		\ba
	          	F_{\mcy,c}^*(\bs{u}) &= 1-\frac{1}{\beta} + \frac{1}{\beta}\min\left\{ \min\left\{ \frac{u_t}{2 v_c Y_t \beta }, 1 \right\} \right\}_{t \in \mct} \\
        		\ea
    	\ee
    	for any $c \in \mcc$ and $\bu\in\Rp^T$. If $\beta(\bX,\bY) > 1$, then
	\be
	        \ba
	            F_{\mcy,c}^*(\bs{u}) &= \min\left\{ \min\left\{ \frac{u_t}{2 v_c Y_t  }, 1 \right\} \right\}_{t \in \mct} \\
	        \ea
	\ee
	for any $c \in \mcc$ and $\bu\in\Rp^T$.
\end{lemma}
\begin{proof}
	The minimizing $\dy^*$ is given by
	\be
		\dy^* =
		\begin{cases}
			\frac{1}{\beta}, &\text{if } \beta \leq 1 \\
			1, &\text{if } \beta > 1 \\
		\end{cases}
	\ee
	which yields $\UB_\WC(\dy^*) = L(\beta)$. The form of the strategy $F_\mcy^*$ follows from \eqref{eq:CAS_X} (Definition \ref{def:CAS_X}).
\end{proof}



The next result establishes a lower bound. 

\begin{lemma}\label{lem:LB_WC}
    Consider $\ML(\bX,\bY;W_\WC,\bv)$. Suppose $\hat{F}_\mcx \in \F_\WC(\bX)$ is a strategy of the form \eqref{eq:CAS_X}. Then it holds that for any $F_\mcy \in \F(\bY)$,
    \be
        \pi_\mcx(\hat{F}_\mcx,F_\mcy) \geq \LB_\WC(\dx)
    \ee
    where $\dx \in [0,1]$ is the parameter of $\hat{F}_\mcx$, and
    \be
    	\LB_\WC(\dx) \triangleq \dx\left(1 - \frac{\dx}{2}\beta(\bX,\bY) \right)
    \ee
\end{lemma}
We omit the proof of this result since it follows almost identical logic to the proof of Lemma \ref{lem:UB_WC}. The greatest lower bound can then be easily determined in the following result.

\begin{lemma}\label{lem:max_LB_WC}
	Consider $\ML(\bX,\bY;W_\WC,\bv)$. Then,
	\be\label{eq:LB_OPT_WC}
		\max_{\dx \in [0,1]  } \LB_\WC(\dx) = L(\beta(\bX,\bY)).
	\ee
	The strategy $F_\mcx^* \in \F_\WL(\bX)$ that ensures the lower bound $L(\beta(\bX,\bY))$ is given as follows. 
	If $\beta(\bX,\bY) \leq 1$, then
    	\be
       		\ba
	          	F_{\mcx,c}^*(\bs{u}) &= \min\left\{ \min\left\{ \frac{u_t}{2 v_c X_t }, 1 \right\} \right\}_{t \in \mct} \\
        		\ea
    	\ee
    	for any $c \in \mcc$ and $\bu\in\Rp^T$. If $\beta(\bX,\bY) > 1$, then
	\be
	        \ba
	            F_{\mcx,c}^*(\bs{u}) &= 1-\frac{1}{\beta} +\frac{1}{\beta} \min\left\{ \min\left\{ \frac{u_t}{2 v_c X_t \beta }, 1 \right\} \right\}_{t \in \mct} \\
	        \ea
	\ee
	for any $c \in \mcc$ and $\bu\in\Rp^T$.
\end{lemma}
\begin{proof}
	The minimizing $\dx^*$ is given by
	\be
		\dx^* =
		\begin{cases}
			1 , &\text{if } \beta \leq 1 \\
			\frac{1}{\beta}, &\text{if } \beta > 1 \\
		\end{cases}
	\ee
	which yields $\LB_\WC(\dx^*) = L(\beta)$. The form of the strategy $F_\mcy^*$ follows from \eqref{eq:CAS_X} (Definition \ref{def:CAS_X}).
\end{proof}


We are now ready to establish the main result, Theorem \ref{thm:WL}.

\begin{proof}[Proof of Theorem \ref{thm:WC}]
	From Lemmas \ref{lem:min_UB_WC} and \ref{lem:max_LB_WC}, we obtain
	\be
		\pi_\mcx(F_\mcx,F_\mcy^*) \leq L(\beta) \leq \pi_\mcx(F_\mcx^*,F_\mcy) 
	\ee
	for all $F_\mcx \in \F(\bX)$ and $F_\mcy \in \F(\bY)$. They also imply that $\pi_\mcx(F_\mcx^*,F_\mcy^*) = L(\beta)$. Thus, the strategy profile $(F_\mcx^*,F_\mcy^*)$ is an equilibrium (Definition \ref{def:equil}).
\end{proof}
